Who Are We Missing? A Principled Approach to Characterizing the Underrepresented Population

Randomized controlled trials (RCTs) serve as the cornerstone for understanding causal effects, yet extending inferences to target populations presents challenges due to effect heterogeneity and underrepresentation. Our paper addresses the critical issue of identifying and characterizing underrepresented subgroups in RCTs, proposing a novel framework for refining target populations to improve generalizability. We introduce an optimization-based approach, Rashomon Set of Optimal Trees (ROOT), to characterize underrepresented groups. ROOT optimizes the target subpopulation distribution by minimizing the variance of the target average treatment effect estimate, ensuring more precise treatment effect estimations. Notably, ROOT generates interpretable characteristics of the underrepresented population, aiding researchers in effective communication. Our approach demonstrates improved precision and interpretability compared to alternatives, as illustrated with synthetic data experiments. We apply our methodology to extend inferences from the Starting Treatment with Agonist Replacement Therapies (START) trial -- investigating the effectiveness of medication for opioid use disorder -- to the real-world population represented by the Treatment Episode Dataset: Admissions (TEDS-A). By refining target populations using ROOT, our framework offers a systematic approach to enhance decision-making accuracy and inform future trials in diverse populations.

==> challenges.tex <==
\subsection{Challenges}
Many approaches, including the ones discussed here, use the information from the trial data to generalize treatment effect estimates to the observational sample. Here, the observational sample lacks any information about the outcomes as well as treatment assignment. We only use the pre-treatment covariates from the observational data to understand the distribution shift between the trial and the observational data, and appropriately adjust for it. All the information about the outcomes as well as the treatment effects is solely from the trial cohort. Thus, in cases where there is treatment effect heterogeneity as a function of the pretreatment covariates, if certain combinations of covariate values are under-represented in the trial data compared to the observational sample then their treatment effect estimates are highly imprecise. To a reader, familiar with observational causal inference, this is akin to scenarios where there is limited overlap between the treated and the control samples, making them incomparable to each other. However, there is one major difference. While in observational causal studies, we observe the outcome information under both the treatment arms, here we only observe the outcome information under one study sample, the trial data. 

In what follows, we discuss what this distinction is interesting as well as challenging. Our approach to dealing with the ``lack of positivity'' is similar to the approach discussed in \cite{crump2009dealing} and \cite{li2019addressing}. In their approach, they are interested in estimating the average treatment effect (ATE) -- $\theta := \E_\bX[\tau(\bX)] = \E_\bX[Y(1) - Y(0) \mid \bX]$ -- using only the observational data where they observe the pretreatment covariates ($\bX$), treatment assignment ($T$), and outcomes ($Y$) for each unit. Their approach mainly focuses on redefining the estimand of interest as a reweighted version of the ATE where the weights are functions of the pretreatment features -- $\theta_w = \E_\bX[w(\bX) \tau(\bX)] = \E_\bX[w(\bX) ( Y(1) - Y(0) ) \mid \bX]$. Choosing these weights to be binary indicates if a certain subspace must be included in the analysis or not. To consistently estimate ATE, one requires overlap only in the subspace of common ``confounder'' i.e. the covariates that simultaneously affect $T$ and $Y$. As the outcome is observed in both the treatment arms, it is feasible to identify 

==> introduction.tex <==
\section{Introduction}
Randomized controlled trials (RCTs) are the gold standard for estimating the causal effects of interventions and informing decision-making \citep{ding2023first}. However, a challenge can lie in extending the inferences from trials to target populations, particularly in the face of effect heterogeneity \citep{degtiar2023review, rudolph2023efficiently}. Prior research underscores that the generalizability of RCT evidence to the target population depends on the alignment of distributions of individuals' characteristics - in particular, effect moderators - between the trial cohort and the target population relevant for decision-making. Differences in distributions can compromise treatment effect extrapolations, especially for groups underrepresented in trials, potentially leading to inaccuracies and incorrect decision-making \citep{bell2016, olsen2013, imai2008, pearl2011, pearl2014, bareinboim2014}. It can be particularly hard to identify when such misalignment exists in high-dimensional settings. Crucially, comparability primarily matters for moderators (also known as causal effect modifiers), but identifying which characteristics are moderators can be challenging.

Concerns about the potential lack of representativeness of trial participants have been raised in studies of emergency contraception \citep{glasier2011can}, education \citep{tipton2018review}, substance use \citep{rudolph2022under}, etc.
For example, \cite{glasier2011can} demonstrated that the risk of becoming pregnant for obese women was over threefold higher compared to women with a normal body mass index (BMI). Yet, individuals with a high BMI were frequently underrepresented in emergency contraception clinical trials. Consequently, decisions informed by these trials placed them at an unwarranted risk of pregnancy, highlighting the real-world implications of underrepresentation in clinical trials. Similarly, recent literature underscores the challenges posed by underrepresentation and calls for trials that more accurately represent diverse populations \citep{boden2022confronting, bierer2022advancing, rudolph2022under}. However, as discussed earlier, in practical terms, determining which features to prioritize and identifying underrepresented subgroups remains a complex challenge.

\paragraph{Contribution.} Our work proposes a principled approach to identify underrepresented groups for whom a trial yields insufficient information regarding treatment effect estimates. Once identified, the target population can be refined by removing underrepresented groups, ensuring a more precise estimate of treatment effects and clarity regarding the groups to whom generalization is -- or isn't -- warranted. Our framework translates the objective to an optimization problem that learns the target subpopulation distribution that minimizes the variance of the target average treatment effect (TATE) estimate. We introduce a nonparametric functional optimization approach, Rashomon Set of Optimal Trees (ROOT)\footnote{Rashomon is a classic Japanese movie in which an event is given more than one and often a competing interpretation by the individuals involved. It provides different and sometimes contradictory points of view on the same event. Here, each of the trees in the set provides almost equally good but the different characterization of underrepresented subpopulations -- thus we refer to this set as a Rashomon Set. Analogously, there is also literature in Interpretable Machine Learning that focuses on understanding the properties and behavior of almost equally good but different models \citep{breiman2001statistical, semenova2022existence}.}, to solve the optimization problem. We ensure the output of ROOT is interpretable, enabling researchers to effectively communicate the characteristics of the study population as well as the underrepresented groups. This can inform where the trial inferences can be most precisely extended as well as alert those who may use the trial study results to particular subpopulations underrepresented in the current study. We rigorously evaluated our approach through synthetic data experiments involving complex data-generative procedures with non-linear relationships. We compared the performance of our optimization approach against simpler alternatives. Our findings demonstrate that our approach is efficient in improving precision and yields interpretable results.

We apply our approach to 1) identify underrepresented groups in an RCT of medication for opioid use disorder (MOUD), and 2) extend inferences from that trial to a refined target population that removes these underrepresented groups. This motivating example is of interest, because, although MOUD (methadone, buprenorphine, and extended-release naltrexone) are effective in reducing the risk of opioid overdose, their effect sizes estimated in trials are generally appreciably larger in trials than observed in real-world clinical scenarios \citep{rudolph2022under, susukida2016assessing, blanco2017toward}, and it is important to understand why. We hypothesize that a portion of this incongruity stems from differences between the individuals in the trials and the broader population of patients treated for opioid use disorder. Specifically, we consider the Starting Treatment with Agonist Replacement Therapies (START) MOUD trial \citep{saxon2013buprenorphine}, which compares methadone with buprenorphine; and the real-world population of people for whom MOUD is part of their treatment plan, using the Treatment Episode Dataset: Admissions (TEDS-A) \citep{abuse2020treatment}, which includes all people treated for substance use disorders at programs across the United States that receive public funding.

\paragraph{Paper Organization.} We first summarize the relevant literature in Section~\ref{sec: literature}. In Section~\ref{sec: prelim}, we introduce our setup and assumptions. We propose our framework and the ROOT approach in Sections~\ref{sec: framework} and \ref{sec: method}. %ROOT constructs an ensemble of random trees to determine the optimal function for assigning weights to generalize the trial sample to the refined target population.
We then proceed to demonstrate the effectiveness of our approach through synthetic data experiments in Section~\ref{sec: synth_exp}. Lastly, in Section~\ref{sec: moud}, we discuss the application of our methodology to the MOUD case study. We end with a discussion of the limitations of our approach, posing open questions and future directions (Section~\ref{sec: conclude}).
